Holoported Characters: Real-time Free-viewpoint Rendering of Humans from Sparse RGB Cameras

We present the first approach to render highly realistic free-viewpoint videos of a human actor in general apparel, from sparse multi-view recording to display, in real-time at an unprecedented 4K resolution. At inference, our method only requires four camera views of the moving actor and the respective 3D skeletal pose. It handles actors in wide clothing, and reproduces even fine-scale dynamic detail, e.g. clothing wrinkles, face expressions, and hand gestures. At training time, our learning-based approach expects dense multi-view video and a rigged static surface scan of the actor. Our method comprises three main stages. Stage 1 is a skeleton-driven neural approach for high-quality capture of the detailed dynamic mesh geometry. Stage 2 is a novel solution to create a view-dependent texture using four test-time camera views as input. Finally, stage 3 comprises a new image-based refinement network rendering the final 4K image given the output from the previous stages. Our approach establishes a new benchmark for real-time rendering resolution and quality using sparse input camera views, unlocking possibilities for immersive telepresence.

==> figures/4_hands.tex <==
\begin{figure}
\centering
  \includegraphics[width=\linewidth]{images/4_hands.png}
  \vspace{-24pt}
  \caption{
  %
  \textbf{Recovery of the Hand.}
  %
  Due to our dedicated hand modeling, our method more precisely matches the ground truth hand geometry compared to the baseline.
  %
  }
\label{fig:4_hands}
\end{figure}

==> figures/additional_comparison.tex <==
\begin{figure}
\centering
    %
    \includegraphics[width=1.\linewidth]{images/MoreComparison.png}
    %
    \vspace{-24pt}
    \caption{
    %
    \textbf{Additional Comparison with Other Subjects}
    %
  .
    %
    }
    %
    \label{fig:additonal_comp}
\end{figure}

==> tables/0_comparison_np.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{table*}[b]
\begin{center}
%
\caption
{
Comparison of our method with existing approaches on \textit{novel pose synthesis} on subjects \textit{S1} and \textit{S2}.
Among real-time image driven methods, our results are the most realistic with higher LPIPS and FID metrics.
Results are highlighted as \textbf{best} and \underline{second best} for each metric.
%
}
\vspace{-6pt}
\label{tab:comparison_np}	
\begin{tabular}{@{}cc|ccc|ccc@{}}
    %
    \toprule
    %
    &  & \multicolumn{3}{c|}{Subject S1} & \multicolumn{3}{c}{Subject S2} \\
     \midrule
                                 \textbf{Method}    &\textbf{Real-time} & \textbf{PSNR}$\uparrow$  & \textbf{LPIPS}$\downarrow$ \footnotesize{($\times 1000$)} & \textbf{FID}$\downarrow$ & \textbf{PSNR}$\uparrow$  & \textbf{LPIPS}$\downarrow$ \footnotesize{($\times 1000$)} & \textbf{FID}$\downarrow$  \\
    %
    \midrule
    %
    Neural Actor        &   \cxmark  &    28.43           &    28.33              &    24.50           &    24.78           &    47.15              &    85.87  \\ 
    HDHumans	        &   \cxmark   &    27.69         &    \textbf{24.0}             &     \textbf{9.25}   &   26.32         &   \underline{33.33}             &     \textbf{11.87}        \\
    % TAVA	            &    ???          &    ???             &     ???         \\
    \midrule
    DDC	                &   \ccmark   &    28.05           &    30.43            &    38.37      &    25.92          &    41.07             &     56.43      \\ 
    ENeRF	            &  \ccmark   &    \underline{30.54}    &    29.41             &     36.39      &    \textbf{29.61}         &    36.08             &     41.08   \\
    DVA	                &  \ccmark   &    \textbf{30.60}       &    29.41             &     43.11   &    24.06          &    45.73            &     142.07       \\
    \midrule
    \textbf{Ours}	    &  \ccmark   &   30.19                &  \underline{24.95}        &   \underline{12.80}        &    \underline{28.03}          &   \textbf{28.49}            &     \underline{13.26}    \\ 
    \bottomrule
    %
\end{tabular}
\end{center}
%
\end{table*}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
